Hadron interactions and cosmic strings from lattice simulations

This doctoral thesis focuses on the application of lattice techniques to study two separate topics: hadron interactions within quantum chromodynamics (QCD), and the emission of particles and gravitational waves (GWs) from cosmic string loops. The first part of the dissertation deals with the study of two- an three-particle interactions using lattice QCD simulations, complemented by the limit of large number of colors and chiral perturbation theory. In particular, this part presents results on the study of meson interactions as a function of the number of colors, three-pion interactions in chiral perturbation theory, and two- and three-particle scattering in the (1+1)-dimensional O(3) non-linear sigma model. The second part of the thesis is devoted to the study of the dynamics and decay into particles and GWs of cosmic string loops, using classical-field-theory lattice computations. Results are presented for both global and local string loops.

==> Chapters/Chapter_5/figures/K0K1chpt.tex <==
\begin{figure}[t!]
    \centering
    %
    \begin{subfigure}{0.75\textwidth}
    \centering
        \begin{tikzpicture}
            \begin{axis}[
         		fit plot,
                xlabel={$(\Mpi/\Fpi)^4$}, 
                ylabel={$\displaystyle\frac{\Kiso}{10^3}$}, ylabel shift=0.2ex,
                ymin=-.4, ymax=1.79, ytick distance=.5, restrict y to domain=-1:2,
                xmin=-0.01, xmax=159.9, xtick distance=50, restrict x to domain=-1:180,
                legend pos = north east
                ]
    
                \addplot[LOline, mark=none] 
                    table[x index=0, y index=1, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};

                \addplot[NLOline, mark=none, filled legend] 
                    table[x index=0, y index=2, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};
                \addplot[NLOupperline, mark=none, name path global=NLOU,draw=none] 
                    table[x index=0, y index=3, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};
                \addplot[NLOlowerline, mark=none, name path global=NLOL,draw=none] 
                    table[x index=0, y index=4, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};
                    
                \addplot[Fitline, mark=none, filled legend with mark] 
                    table[x index=0, y index=5, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};
                \addplot[Fitupperline, mark=none, name path global=FitU,draw=none] 
                    table[x index=0, y index=6, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};
                \addplot[Fitlowerline, mark=none, name path global=FitL,draw=none] 
                    table[x index=0, y index=7, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K0data.txt};
                    
                \addplot [fitorange, opacity=0.3] fill between[of=FitU and FitL];
                \addplot [fitgray, opacity=0.3] fill between[of=NLOU and NLOL];
                
    			\addplot [lattice data=fitorange]
               	table [x index = 0, y index = 1, x error index = 2, y error index = 3]
               	{Chapters/Chapter_5/figures/data/K0points.txt};        
               	
               	\addplot[zeroline] coordinates {(-1,0) (170,0)};
                        
                \legend{\small LO ChPT,\small LO+NLO ChPT,,,\small {\fakeblanton\ and LO+NLO fit}}
    		
    		\end{axis}
        \end{tikzpicture}
    \end{subfigure}%

    \begin{subfigure}{0.75\textwidth}
    \centering
        \begin{tikzpicture}
            \begin{axis}[
         		fit plot,
                xmin=-0.01, xmax=159.9, xtick distance=50, restrict x to domain=-1:180,     
                ymin=-2.9, ymax=2.31, ytick distance=1, restrict y to domain=-4:4,
                xlabel={$(\Mpi/\Fpi)^4$},       
                ylabel={$\displaystyle\frac{\Kisoone}{10^3}$},
                legend pos = north east,
                y tick label style={
                /pgf/number format/.cd,
                fixed,
                precision=0,
                /tikz/.cd
                },
                ]
    
                \addplot[LOline, mark=none] 
                    table[x index=0, y index=1, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                    
                \addplot[NLOline, mark=none, filled legend] 
                    table[x index=0, y index=2, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                \addplot[NLOupperline, mark=none, name path global=NLOU,draw=none] 
                    table[x index=0, y index=3, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                \addplot[NLOlowerline, mark=none, name path global=NLOL,draw=none] 
                    table[x index=0, y index=4, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                    
                \addplot[Fitline, mark=none, filled legend with mark] 
                    table[x index=0, y index=5, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                \addplot[Fitupperline, mark=none, name path global=FitU,draw=none] 
                    table[x index=0, y index=6, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                \addplot[Fitlowerline, mark=none, name path global=FitL,draw=none] 
                    table[x index=0, y index=7, col sep=tab] 
                    {Chapters/Chapter_5/figures/data/K1data.txt};
                    
                \addplot [fitorange, opacity=0.3] fill between[of=FitU and FitL];
                \addplot [fitgray, opacity=0.3] fill between[of=NLOU and NLOL];
                
                \addplot [scatter, only marks, mark=*, scatter/use mapped color={draw=fitorange,fill=orange}, mark options={scale=0.7}]
               	table [x index = 0, y index = 1]
               	{Chapters/Chapter_5/figures/data/K1points.txt};
    
    			\addplot [lattice data=fitorange]
               	table [x index = 0, y index = 1, x error index = 2, y error index = 3]
               	{Chapters/Chapter_5/figures/data/K1points.txt};  
               	
               	\addplot[zeroline] coordinates {(-1,0) (170,0)};             
    
                \legend{\small LO ChPT,\small LO+NLO ChPT,,,\small {\fakeblanton\ and LO+NLO fit}}
            \end{axis}
           
        \end{tikzpicture}
    \end{subfigure}

    \caption[]{
        LO (dashed black line) and LO+NLO (grey line and band) ChPT predictions for $\Kiso$ (top) and $\Kisoone$ (bottom) as functions of $(\Mpi/\Fpi)^4$, using LECs from \rrcite{Colangelo:2001df,FLAG:2021npn} [see \cref{eq:pipipiKmatrix:LECref}].
        These predictions are compared to lattice results from \rcite{Blanton:2021llb} (orange points).
        We also present the best fit to the lattice data (dotted orange line and orange band).}
\label{fig:pipipiKmatrix:K0K1chpt}
\end{figure}

==> Chapters/Chapter_6/figures/DiagramAll.tex <==
\begin{figure}[thp]
    \begin{multline*}
            \tikzineq[xscale=1.5,yscale=1.5]{
                \makeexternallegcoordinates
                \coordinate (v) at (0,0);
                \draw[sketch onshell prop] (k1) -- (v);
                \draw[sketch onshell prop] (k2) -- (v);
                \draw[sketch onshell prop] (k3) -- (v);
                \draw[sketch onshell prop] (v) -- (p1);
                \draw[sketch onshell prop] (v) -- (p2);
                \draw[sketch onshell prop] (v) -- (p3);
                \node[sketch onshell blob=NLOcolor, inner sep=-3pt]
                    (M) at (0,0) {\footnotesize $\Mdf^\NLO$};
            }
        \quad\scalebox{\sketchoperatorscale}{$\bm=$}\quad
        \quad
        \underset{\rule{0pt}{1.5em}\displaystyle\cM^{\NLO,\OPE}}{%
            \tikzineq[xscale=1.5,yscale=1.2]{
                \makeexternallegcoordinates
                \coordinate (v1) at (+.4,-.5);
                \coordinate (v2) at (-.4,+.5);
                \draw[sketch onshell prop] (k1) -- (v2);
                \draw[sketch onshell prop] (k2) -- (v1) -- (k3);
                \draw[sketch onshell prop] (p3) -- (v1);
                \draw[sketch onshell prop] (p1) -- (v2) -- (p2);
                \draw[sketch offshell prop] (v1) -- (v2);
                \node[sketch offshell blob=NLOcolor, inner ysep=2pt, inner xsep=-1pt]
                    (NLO) at (v1) {\scalebox{.7}{$\cM_2^{\NLO,\off}$}};
                \node[sketch offshell blob=LOcolor, inner ysep=2pt, inner xsep=-1pt]
                    (LO) at (v2) {\scalebox{.7}{$\cM_2^{\LO,\off}$}};
            }
        }
        \quad\scalebox{\sketchoperatorscale}{$\bm-$}\quad
        \underset{\rule{0pt}{1.5em}\displaystyle\cD^{\NLO,\OPE}}{%
            \tikzineq[xscale=1.5,yscale=1.2]{
                \makeexternallegcoordinates
                \coordinate (v1) at (+.4,-.5);
                \coordinate (v2) at (-.4,+.5);
                \draw[sketch onshell prop] (k1) -- (v2);
                \draw[sketch onshell prop] (k2) -- (v1) -- (k3);
                \draw[sketch onshell prop] (p3) -- (v1);
                \draw[sketch onshell prop] (p1) -- (v2) -- (p2);
                \draw[sketch offshell prop] (v1) -- (v2);
                \node[sketch onshell blob=LOcolor, inner sep=0pt]
                    (LO) at (v2) {\scalebox{.7}{$\cM_2^{\LO}$}};
                \node[sketch onshell blob=NLOcolor, inner sep=-2pt]
                    (NLO) at (v1) {\scalebox{.7}{$\cM_2^{\NLO}$}};
            }
        }\\
        \quad\scalebox{\sketchoperatorscale}{$\bm+$}\;\,
        \underset{\rule{0pt}{1.5em}\displaystyle\cM_3^{\NLO,\nonOPE}}{%
            \tikzineq[xscale=1.5,yscale=1.5]{
                \makeexternallegcoordinates
                \coordinate (v) at (0,0);
                \draw[sketch onshell prop] (k1) -- (v);
                \draw[sketch onshell prop] (k2) -- (v);
                \draw[sketch onshell prop] (k3) -- (v);
                \draw[sketch onshell prop] (v) -- (p1);
                \draw[sketch onshell prop] (v) -- (p2);
                \draw[sketch onshell prop] (v) -- (p3);
                \node[sketch onshell blob=NLOcolor, inner sep=0pt]
                    (M) at (0,0) {\footnotesize $A^{(4)}$};
            }
        }
        \quad\scalebox{\sketchoperatorscale}{$\bm-$}\quad
        \underset{\rule{0pt}{1.5em}\displaystyle\cD^\BH}{%
            \tikzineq[xscale=2,yscale=1.5]{
                \makeexternallegcoordinates
                \coordinate (v1) at (+.5,+.4);
                \coordinate (v2) at (-.5,+.4);
                \coordinate (v3) at (  0,-.6);
                \draw[sketch onshell prop] (k1) -- (v1);
                \draw[sketch onshell prop] (k2) -- (v1);
                \draw[sketch onshell prop] (k3) -- (v3);
                \draw[sketch onshell prop] (v2) -- (p1);
                \draw[sketch onshell prop] (v2) -- (p2);
                \draw[sketch onshell prop] (v3) -- (p3);
                \draw[sketch onshell prop] (v1) -- (v2);
                \draw[sketch offshell prop] (v1) -- (v3);
                \draw[sketch offshell prop] (v2) -- (v3);
                \foreach \i in {1,2,3}
                    \node[sketch onshell blob=LOcolor, inner sep=-1pt]
                        (M\i) at (v\i) {\scalebox{.7}{$\cM_2^\LO$}};
            }
        }
        \quad\scalebox{\sketchoperatorscale}{$\bm+$}\quad
        \underset{\rule{0pt}{1.5em}\displaystyle\cM^{\NLO,\sOPE}}{%
            \tikzineq[xscale=1.8,yscale=1.2]{
                \makeexternallegcoordinates
                \coordinate (v1) at (+.5,0);
                \coordinate (v2) at (-.5,0);
                \draw[sketch onshell prop] (k1) -- (v1);
                \draw[sketch onshell prop] (k2) -- (v1) -- (k3);
                \draw[sketch onshell prop] (p3) -- (v2);
                \draw[sketch onshell prop] (p1) -- (v2) -- (p2);
                \draw[sketch offshell prop] (v1) -- (v2);
                \node[sketch offshell blob=NLOcolor, inner ysep=2pt, inner xsep=-1pt]
                    (NLO) at (v1) {\scalebox{.7}{$\cM_2^{\NLO,\off}$}};
                \node[sketch offshell blob=LOcolor, inner ysep=2pt, inner xsep=-1pt]
                    (LO) at (v2) {\scalebox{.7}{$\cM_2^{\LO,\off}$}};
            }
        }
    \end{multline*}
    \caption{
        Schematic representation  of \cref{eq:mastereq}, which extends \cref{fig:pipipiKmatrix:diagram} to general isospin.
        As in \cref{fid:pipipiKmatrix:diagram}, solid and dotted lines represent on- and off-shell pions, respectivey.
        Square boxes indicate fully on-shell amplitudes, while oval boxes have one leg off shell.
        Finally, blue and pink fillings indicate, LO and NLO quantities, in this same order.
        For the $\OPE$ and $\sOPE$ contributions, there are additional diagrams  in which the $\LO$ and $\NLO$ amplitudes are exchanged.}
    \label{fig:isospinKmatrix:NLOseparation}
\end{figure}

